Neural calibration of hidden inhomogeneous Markov chains -- Information decompression in life insurance

Markov chains play a key role in a vast number of areas, including life insurance mathematics. Standard actuarial quantities as the premium value can be interpreted as compressed, lossy information about the underlying Markov process. We introduce a method to reconstruct the underlying Markov chain given collective information of a portfolio of contracts. Our neural architecture explainably characterizes the process by explicitly providing one-step transition probabilities. Further, we provide an intrinsic, economic model validation to inspect the quality of the information decompression. Lastly, our methodology is successfully tested for a realistic data set of German term life insurance contracts.

==> Plots/female_error_rel_stats.tex <==
\begin{tabular}{lrrrrrrrrr}
\toprule
{} &  0.000 &  0.005 &  0.100 &  0.250 &  0.500 &  0.750 &  0.900 &  0.995 &  1.000 \\
\midrule
female \$q\_\textbackslash alpha\$ [\%] &  -8.62 &  -5.69 &  -2.98 &  -1.38 &  -0.18 &   0.86 &   1.91 &   4.38 &   5.96 \\
\bottomrule
\end{tabular}

